Deduplicator: When Computation Reuse Meets Load Balancing at the Network Edge

Load balancing has been a fundamental building block of cloud and, more recently, edge computing environments. At the same time, in edge computing environments, prior research has highlighted that applications operate on similar (correlated) data. Based on this observation, prior research has advocated for the direction of "computation reuse", where the results of previously executed computational tasks are stored at the edge and are reused (if possible) to satisfy incoming tasks with similar input data, instead of executing incoming tasks from scratch. Both load balancing and computation reuse are critical to the deployment of scalable edge computing environments, yet they are contradictory in nature. In this paper, we propose the Deduplicator, a middlebox that aims to facilitate both load balancing and computation reuse at the edge. The Deduplicator features mechanisms to identify and deduplicate similar tasks offloaded by user devices, collect information about the usage of edge servers' resources, manage the addition of new edge servers and the failures of existing edge servers, and ultimately balance the load imposed on edge servers. Our evaluation results demonstrate that the Deduplicator achieves up to 20% higher percentages of computation reuse compared to several other load balancing approaches, while also effectively balancing the distribution of tasks among edge servers at line rate.

==> sections/discussion.tex <==
\section {Discussion}
\label{sec:discussion}

\noindent\textbf{Fault tolerance:} Since the \sol is responsible for distributing incoming tasks based on the slices of the hash space assigned to the available edge servers, it can become a single point of failure. To increase the reliability of the whole system, multiple instances of the \sol can be deployed. When deploying multiple \sol instances, it is important to maintain the consistency of the hash space slices assigned to edge servers. The configuration of these instances can be either an active-passive or an active-active~\cite{eisenbud2016maglev, levin2018hierarchical}. In an active-passive configuration, one of the \sol instances will be active (\ie distributes the load among the available edge servers) while other instances remain in standby mode. On the other hand, in an active-active configuration, multiple instances of the \sol are simultaneously active and together distribute incoming tasks. 


\noindent\textbf{Deciding on appropriate similarity thresholds for reuse:} For a particular application, the application developer or the service provider can select an approximate initial value for the similarity threshold (based on the nature of the application). The edge servers will initially reuse computation based on this approximate similarity threshold, and the \sol will adjust the threshold value by sampling the reuse accuracy of groups of tasks over time. The sampling process can take place by having edge servers execute from scratch small groups of tasks $g_1, g_2, ..., g_n$ for which they have results that they could potentially reuse and compare the results of the execution of $g_1, g_2, ..., g_n$ with the results of the tasks that could be reused. Based on this process, the \sol can estimate the reuse accuracy and adjust the similarity threshold accordingly. 

%For the sampling, the \sol can ask the edge servers to additionally execute a few tasks from scratch for which the results are reused. And the edge servers provide both the executed results and the reused results to the \sol. Based on these results, the \sol can get an approximate idea of the reuse accuracy and fine-tune the similarity threshold accordingly. However, this fine-tuning approach will cause some additional overhead to the \sol and edge servers.  

\noindent\textbf{Security and privacy considerations:} Identifying tasks with similar input data can inadvertently have security and privacy implications. In the case of user assisted hashing, the input data can be encrypted and the \sol can only see the LSH value of the input data. Additionally, differential privacy can be utilized to preserve the privacy of input data by adding carefully calibrated noise to the LSH function~\cite{fernandes2021locality}. Since the noise will be carefully calibrated, it will allow the \sol to identify tasks with similar input data based on the LSH value while making it difficult to infer specific information about the input data from the LSH value. 

%\noindent\textbf{Controlling the granularity of the slices:} To adjust the granularity of the slices, we employed a dynamic binning approach, which allows to change the slice sizes more flexibly with less overhead. In this approach, the whole hash space is divided into a certain number of fixed-size bins and each slice can contain multiple bins (typically consecutive bins). The \sol keeps track of how many requests has been forwarded for each bin. And whenever the redistribution or adjustment of the hash space is required, the \sol uses this bin-specific information. As a results. the slices assigned to the available edge server can be adjusted to be more fine-grained or coarse-grained efficiently. 

\begin{comment}
\begin{itemize}
    \item similarity threshold
    \item what if the load balancer fails -- Yoda \cite{gandhi2016yoda} like scale-out approaches to avoid a single point of failure 
    \item what happens when a backend is added or removed -- should not impact all the servers 
\end{itemize}
\end{comment}
